B, D and K decays

With the advent of the LHC, we will be able to probe New Physics (NP) up to energy scales almost one order of magnitude larger than it has been possible with present accelerator facilities. While direct detection of new particles will be the main avenue to establish the presence of NP at the LHC, indirect searches will provide precious complementary information, since most probably it will not be possible to measure the full spectrum of new particles and their couplings through direct production. In particular, precision measurements and computations in the realm of flavour physics are expected to play a key role in constraining the unknown parameters of the Lagrangian of any NP model emerging from direct searches at the LHC. The aim of Working Group 2 was twofold: on one hand, to provide a coherent, up-to-date picture of the status of flavour physics before the start of the LHC; on the other hand, to initiate activities on the path towards integrating information on NP from high-pT and flavour data.

==> actions-ref.tex <==
jonas check ref `
\bibitem {vava-lhcb1} V Gligorov, J Rademacker. Correcting for trigger biases
in lifetime fitting at LHCb. September 2006. NOTE LHCB-??.

is this actually
 Monte Carlo independent lifetime fitting at LHCb in lifetime biased channels
CERN-LHCb-2007-053, 06/06/2007, by V. Gligorov, J. Rademacker
 

marco ciuchini
in preparation b2sandb2d

Hazumi, ICHEP 2006


Although the result for each individual mode
does not significantly differ from
the SM expectation (i.e. $\cals_{\jpsi\kz}$),
all the $\cals$ values are smaller
than the SM expectation.
When all the $b\to s$ modes are combined,
the result differs from the SM expectation
by 2.6$\sigma$.
Much more data are needed to firmly establish
a new $CP$-violating phase beyond the SM
for each golden mode.


Although the result for each individual mode
does not significantly differ from
the SM expectation (i.e. $\cals_{\jpsi\kz}$),
%all the $\cals$ values are smaller
%than the SM expectation.
%When all the $b\to s$ modes are combined,
%the result differs from the SM expectation
%by 2.6$\sigma$.
most of the $\cals$ values are smaller
than the SM expectation.
When all the $b\to s$ modes are combined,
the result differs from the SM expectation
by 1.1$\sigma$\footnote{%
Due to the highly non-Gaussian errors of the result from $B^0 \to f_0K^0_S$ 
with $f_0 \to \pi^+\pi^-$, and the fact that this result has a significant effect 
on the $\chi^2$ of the naïve $b\to s$ penguin average, 
this outlying point is excluded.
}
Combining the results of all the $b\to s$ modes 
is naive as the theoretical uncerainties 
vary considerably amongst the modes.
Much more data are needed to firmly establish
a new $CP$-violating phase beyond the SM
for each golden mode.


==> charm/cpvuntagged.tex <==
More importantly, regardless of the theoretical estimates, this strong phase can be 
measured at CLEO-c, so Eq.~(\ref{KpiTime}) depends {\it only} on experimentally-measurable 
quantities. It is also easy to obtain the time-integrated asymmetry for $K\pi$. Neglecting small
subleading terms of ${\cal O}(\lambda^4)$,
%
\beq \label{KpiIntegrated}
%A_{CP}^U (K\pi) = - y \sin \delta \sin \phi \sqrt{R}. 
A_{CP}^U (K\pi) = - y \sin \delta \sin \phi  \left|A_f/\overline{A}_f \right|. 
\eeq
%
It is important to note that both time-dependent and time-integrated asymmetries
of Eqs.~(\ref{KpiTime}) and (\ref{KpiIntegrated}) are independent of predictions
of hadronic parameters, as both $\delta$ and $R$ are experimentally determined 
quantities and could be used for model-independent extraction of CP-violating phase 
$\phi$. Assuming $R \sim 0.4\%$ and $\delta \sim 40^o$~\cite{Falk:1999ts} and
$y \sim 1\%$ one obtains $\left| A_{CP}^U (K\pi) \right| \sim \left(0.04\%\right)\sin\phi$.
For SCS modes, where $R \sim 1$, the resulting asymmetry could be ${\cal O}(1\%)\sin\phi$. 
However, the final states must be chosen such that $A_{CP}^U$ is not trivially zero. For example, 
decays of $D$ into the final states that are CP-eigenstates would result 
in zero asymmetry (as $\Gamma_f=\Gamma_{\overline f}$ for those final states) 
while decays to final states like $K^+ K^{*-}$ or $\rho^+ \pi^-$ would not.
It is also likely that this asymmetry is larger than the estimate given above 
due to contributions from direct CP-violation (see eq.~\ref{Coefficients}). 
The final state $f$ can also be a multiparticle state. In that case,
more untagged CP-violating observables could be constructed~\cite{Petrov:2004gs}.



==> charm/impactB.tex <==
authors: Bigi, Cassel 

==> charm/impactCKM.tex <==
authors: Rosner, Cassel

==> mixing/bsmixing-test.tex <==

\subsection{$B$-meson mixing}

%{\it Coordinators: V. Lubicz, J. van Hunen}

%{\it Authors: P. Ball, M. Bona, S. Burdin, V. Gligorov, D. Guadagnoli, 
%J.J. van Hunen, A. Lenz, V. Lubicz, A. Robert, O. Schneider, L. Silvestrini, 
%M. Smizanska, T. Speer, A. Starodumov, A. Stocchi, S. T'Jampens, V. Vagnoni, 
%Y. Xie}

\subsubsection{Introduction}

During this workshop there has been a breakthrough in the experimental 
study of
\bsmix mixing with the measurement of the following quantities:
the oscillation frequency \dms by the CDF
collaboration~\cite{Abulencia:2006ze}, the time-integrated
untagged charge asymmetry in semileptonic \Bs
decays $A_{SL}^{s,unt}$ and the dimuon asymmetry \asl by
D\O~\cite{Abazov:2007nw,Abazov:2006qw}, the \Bs lifetime from
flavour-specific final 
states~\cite{Barberio:2006bi,Buskulic:1996ei,Abe:1998cj,Abreu:2000sh,
Ackerstaff:1997qi,Abazov:2006cb},
\dgg from the time-integrated angular analysis of $B_s \to J/\psi \phi$ decays
by CDF~\cite{Acosta:2004gt}, supplemented by the three-dimensional constraint 
on $\Gamma_\text{s}$, \dg, and the \bsmix mixing phase from the time-dependent
angular analysis of \bspsiphi decays by D\O~\cite{Abazov:2007tx}.
These measurements can be compared with the Standard Model (SM) predictions and
used to constrain New Physics (NP) contributions to the \bsmix mixing 
amplitude.

In this section we first discuss the
theoretical predictions within the SM and their uncertainties. We then present
the results of a model-independent analysis of NP in \bsmix mixing. We
discuss the implications of the experimental data for SUSY models by either
allowing new sources of flavour and CP violation in the \Bs sector or by
considering a constrained Minimal Flavour Violation SUSY scenario.
The remainder of the section is devoted to the experimental aspects of the 
measurements listed above and gives an outlook for the LHC. 


\subsubsection{Standard model predictions}
\label{sec:SMpredictions}
The neutral $B_d$ and $B_s$ mesons mix with their antiparticles leading to
oscillations between the mass eigenstates. The time evolution of the neutral
meson doublet is described by a Schr\"odinger equation with an effective $2
\times 2$ Hamiltonian
\be
i\frac{d}{dt} \begin{pmatrix} B_q \\ {\bar B}_q \end{pmatrix} =
\left[ 
\begin{pmatrix} M_{11}^q & {M_{12}^q} \\ {M_{12}^q}^* & M_{11}^q\end{pmatrix}
-\frac{i}{2} \begin{pmatrix} \Gamma_{11}^q & {\Gamma_{12}^q} \\
{\Gamma_{12}^q}^* & \Gamma_{11}^q\end{pmatrix} \right]
\begin{pmatrix}B_q\\ {\bar B}_q\end{pmatrix}\,,
\ee
with $q=d,s$. The mass difference $\Delta m_q$ and the width difference $\Delta
\Gamma_q$ are defined as
\be
\Delta m_q=m^q_H-m^q_L\,,\quad
\Delta\Gamma_q=\Gamma^q_L-\Gamma^q_H\,,
\ee
where $H$ and $L$ denote the Hamiltonian eigenstates with the heavier and
lighter mass eigenvalue, respectively. These states can be written as
\be
\vert B_q^{H,L}\rangle =\frac{1}{\sqrt{1+\vert (q/p)_q \vert^2}}\,\left(
\vert B_q\rangle \pm  \left(q/p\right)_q\vert {\bar B}_q\rangle
\right)\,.
\ee

Theoretically, the experimental observables $\Delta m_q$, $\Delta \Gamma_q$ and
$\vert(q/p)_q\vert$ are related to $M^q_{12}$ and $\Gamma^q_{12}$. In the
$B_d-\bar B_d$ and $B_s-\bar B_s$ systems, the ratio $\Gamma^q_{12}/M^q_{12}$ 
is of ${\cal O}(m_b^2/m_t^2)\simeq 10^{-3}$ and, neglecting terms of ${\cal O}
(m_b^4/m_t^4)$, one has
\be
\Delta m_q= 2\,\vert M^q_{12}\vert\,,\quad
\frac{\Delta\Gamma_q}{\Delta m_q}
=-{\mathrm{Re}}\left(\dfrac{\Gamma^q_{12}}{M^{q}_{12}} \right)\,,\quad
1-\left\vert\left(\dfrac{q}{p}\right)_q\right\vert =
\dfrac{1}{2}\,{\mathrm{Im}}
\left( \dfrac{\Gamma^q_{12}}{M^q_{12}}\right)\,.
\ee

The matrix elements $M^q_{12}$ and $\Gamma^q_{12}$ are related to the 
dispersive and the absorptive parts of the $\DB=2$ transitions, respectively. 
Short distance
QCD corrections to these matrix elements have been computed at the NLO for both
$M^q_{12}$~\cite{Buras:1990fn} and
$\Gamma^q_{12}$~\cite{Beneke:1998sy,Beneke:2003az,Ciuchini:2003ww}. The long
distance effects are contained in the matrix elements of four-fermion operators
which have been computed with lattice QCD using various approaches to treat the
$b$ quark 
(HQET, NRQCD, QCD)~\cite{Dalgic:2006gp,Gimenez:2000jj,Hashimoto:2000eh,
Aoki:2002bh,Becirevic:2000sj,Lellouch:2000tw,Yamada:2001xp}. The
corresponding bag parameters $B$ are found to be essentially insensitive to the
effect of the quenched approximation (see sec. \ref{subsec:latqcd}).

The quantity ${\rm Im}(\Gamma^q_{12}/M^q_{12})$ can be measured through the
CP asymmetry in $B_q$ decays to flavour-specific final states.
An important example is the semileptonic asymmetry 
\begin{equation}
A^{s}_{SL}={\rm Im}\left(\frac{\Gamma^q_{12}}{M^q_{12}}\right)=
\frac{N(\bar{B}_{s}\to l^{+} X) - N(B_{s} \to l^{-}
X)}{N(\bar{B}_{s}\to l^{+} X) + N(B_{s} \to l^{-} X)}.
%= \frac{\Delta\Gamma_{s}}{\Delta M_{s}} \tan \phi_{s}.
\label{eq:A_SL_s}
\end{equation}

Two updated theoretical predictions for $\Delta \Gamma_{s}/\Gamma_{s}$ and for
the semileptonic asymmetry $A_{SL}^s$, obtained by
including NLO QCD and ${\cal O}(1/m_b)$~\cite{Beneke:1996gn} corrections, are
\bea
& \Delta \Gamma_{s}/\Gamma_{s} = (7 \pm 3)\cdot 10^{-2} \quad ,
& A_{SL}^s = (2.56 \pm 0.54)\cdot 10^{-5} \quad
\mbox{\cite{Ciuchini:2003ww}} \,, \nn \\
& \Delta \Gamma_{s}/\Gamma_{s} = (13 \pm 2)\cdot 10^{-2} \quad ,
& A_{SL}^s = (2.06 \pm 0.57)\cdot 10^{-5} \quad
\mbox{\cite{Lenz:2006hd}} \,.
\eea
The difference in the central values of $\Delta \Gamma_{s}/\Gamma_{s}$ 
is mainly
due to a different choice of the operator basis~\cite{Lenz:2006hd} and it is
related to unknown ${\cal O}(\alpha_s^2)$ and ${\cal O}(\alpha_s/m_b)$
corrections. Although the basis chosen in ref.~\cite{Lenz:2006hd} leads to
smaller theoretical uncertainties, the shift observed in the central values may
signal that the effect of higher-order corrections on $\Delta \Gamma_{s}
/\Gamma_{s}$ is larger than what could have been previously estimated. We take
into account this uncertainty by quoting, as final theoretical predictions in
the SM, the more conservative estimate~\cite{Tarantino:2007nf}
\be
\Delta \Gamma_{s}/\Gamma_{s} = (11 \pm 4)\cdot 10^{-2} \quad , \quad
A_{SL}^s = (2.3 \pm 0.5)\cdot 10^{-5} ~.
\ee

Concerning $\Delta m_s$, the SM predictions obtained by the UTfit and CKMfitter
Collaborations are
\be
\Delta m_s = (18.4 \pm 2.4)~\mathrm{ps}^{-1} 
\mbox{\cite{Bona:2006ah}} \quad , \quad
\Delta m_s = (18.9^{+5.7}_{-2.8})~\mathrm{ps}^{-1} 
\mbox{\cite{Charles:2004jd}}.
\label{eq:dms-sm}
\ee

\subsubsection{$B_s - \bar B_s$ mixing beyond the SM}
\label{sec:NP}

We now discuss the analysis of $B_s - \bar B_s$ mixing in the presence of
new physics (NP) contributions to the $\DB=2$ effective Hamiltonian.
These can
be incorporated in the analysis in a model independent way, parametrising the
shift induced in the mixing frequency and phase with two parameters, $C_{B_s}$
and $\phi_s\equiv 2\phi_{B_s}$, having in the SM expectation values of 1 and 0,
respectively
\cite{Soares:1992xi,Deshpande:1996yt,Silva:1996ih,Cohen:1996sq,
Grossman:1997dd}:
\be \label{phibsdef}
C_{B_s}  e^{i \phi_s} \equiv C_{B_s}  e^{2 i \phi_{B_s}} =
\frac{\left(M^s_{12}\right)^\mathrm{SM+NP}}
{\left(M^s_{12}\right)^\mathrm{SM}} \, .
\ee

As for the absorptive part of the $B_s -\bar B_s$ mixing amplitude, which is
derived from the double insertion of the $\DB=1$ effective Hamiltonian, it 
could be affected by NP effects in $\DB=1$ transitions through
penguin contributions. Such NP contributions were considered in 
\cite{Bona:2005eu,Bona:2006sa}, but they are not expected to play a dominant
role. We shall neglect them in the present discussion.
In this approximation, which is followd by most authors, NP enters
\bsmix mixing only through the two parameters defined in (\ref{phibsdef}).

Since the SM phase of $\Gamma^s_{12}/M^s_{12}$ is small
in comparison with the current experimental sensitivity, we shall
assume in the following that CP violation in $B_s$ mixing
is dominated by the NP mixing phase $\phi_s$.
We then have 
\begin{equation}\label{alsphis}
A^{s}_{SL}= \frac{\Delta\Gamma_{s}}{\Delta M_{s}} \tan \phi_{s}
\end{equation}
and the same NP phase $\phi_s$ will also govern mixing-induced
CP violation in the exclusive channel \bspsiphi. Note that the phases in 
$A^s_{SL}={\rm Im}(\Gamma^s_{12}/M^s_{12})$ and in the
\bspsiphi asymmetry are different from each other in the SM,
where ${\rm arg}(\Gamma^s_{12}/M^s_{12})\approx 0.004$
while the phase measured in \bspsiphi decay is 
$-2\beta_s\approx -2\lambda^2\eta\approx -0.04$ 
(see e.g. \cite{Lenz:2006hd}).

%As for the absorptive part of the $B_s -\bar B_s$ mixing amplitude, which is
%derived from the double insertion of the $\DB=1$ effective Hamiltonian, it can
%be affected by non negligible NP effects in $\DB=1$ transitions through 
%penguin contributions. Following refs.~\cite{Bona:2005eu,Bona:2006sa}, 
%we thus introduce
%two additional parameters, $C_s^\mathrm{Pen}$ and $\phi_s^\mathrm{Pen}$, which
%encode NP contributions to the penguin part of the $\DB=1$ Hamiltonian, in
%analogy to $C_{B_s}$ and $\phi_{B_s}$ in the $\DB=2$ mixing amplitude.

Making use of the experimental information described in sect.\ref{sec:EXP}, 
it is possible to constrain $C_{B_s}$ and
$\phi_{B_s}$~\cite{Grossman:2006ce,Bona:2005eu,Bona:2006sa,Lenz:2006hd,
Ligeti:2006pm,Ball:2006xx,Bona:2007vi}. We report here the results obtained in
ref.~\cite{Bona:2007vi}.

The use of $\Delta \Gamma_s /\Gamma_s$ from the time-integrated angular 
analysis of $B_s \to J/\psi \phi$ decays is described for instance in
ref.~\cite{Bona:2006sa}. Here we use only the CDF
measurement~\cite{Acosta:2004gt} as input, since the D\O\ analysis is now
superseded by the new time-dependent study~\cite{Abazov:2007tx}.  The latter provides
the first direct constraint on the $B_s$--$\bar B_s$ mixing phase, but also a
simultaneous bound on $\Delta \Gamma_s$ and $\Gamma_s$. The time-dependent
analysis determines the $B_s$--$\bar B_s$ mixing phase with a four-fold
ambiguity. First of all, being untagged, it is not directly sensitive to $\sin
\phi_s$, resulting in the ambiguity $(\phi_s,\cos \delta_{1,2}) \leftrightarrow
(-\phi_s,-\cos \delta_{1,2})$, where $\delta_{1,2}$ represent the strong phase
differences between the transverse polarisation and the other ones. Second, at
fixed sign of $\cos \delta_{1,2}$, there is the ambiguity $(\phi_s,\Delta
\Gamma_s) \leftrightarrow (\phi_s+\pi,-\Delta \Gamma_s)$. One could be tempted
to use factorisation \cite{Lenz:2006hd} or $B_d \to J/\psi K^*$ with SU(3)
\cite{rescigno} to fix the sign of $\cos \delta_{1,2}$. Unfortunately, neither
factorisation nor SU(3) are accurate enough to draw firm conclusions on these
strong phases. This is confirmed by the fact that the two approaches lead to
opposite results. Waiting for future, more sophisticated experimental analyses,
which could resolve this ambiguity with a technique similar to the one used by
BaBar in $B_d \to J/\psi K^*$ \cite{Aubert:2004cp}, we prefer to be 
conservative and keep the four-fold ambiguity.

Compared to previous analyses, the additional experimental input discussed 
below improves considerably the determination of the phase of the 
$B_s - \bar B_s$
mixing amplitude. The fourfold ambiguity inherent in the untagged analysis of
ref.~\cite{Abazov:2007tx} is somewhat reduced by the measurements of $A_{SL}^s$
and $A_{SL}$ (see (\ref{eq:A_SL})), 
which slightly prefer negative values of $\phi_{B_s}$. The results
for $C_{B_s}$ and $\phi_{B_s}$, obtained from the general analysis allowing for
NP in all sectors, are
\be
C_{B_s} = 1.03 \pm 0.29 \quad , \quad
\phi_{B_s}= (-75 \pm 14)^\circ \cup (-19 \pm 11)^\circ \cup (9 \pm 10)^\circ
\cup (102 \pm 16)^\circ ~.
\ee
Thus, the deviation from zero in $\phi_{B_s}$ is below the $1 \sigma$ level,
although clearly there is still ample room for values of $\phi_{B_s}$ very far
from zero. The corresponding p.d.f. in the $C_{B_s}$-$\phi_{B_s}$ plane is
shown in fig.~\ref{fig:cbsphibs}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.45\textwidth]{mixing/PLOTS/cbsvsphibs-np.eps}
\caption{Constraints on  $\phi_{B_s}$ vs. $C_{B_s}$ from the NP generalised
analysis of ref.~\cite{Bona:2007vi}.}
\label{fig:cbsphibs}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{$B_s - \bar B_s$ in SUSY with non-minimal flavour violation}
\label{sec:SUSY}

The results on $C_{B_s}$ and $\phi_{B_s}$ obtained above can be used to
constrain any NP model. As an interesting example we discuss here the case of
SUSY with new sources of flavour and CP violation, following ref.~\cite{vale}.

To fulfill our task in a model-independent way, we use the mass-insertion
approximation to evaluate the gluino mediated contribution to $b\to s$
transitions. Treating off-diagonal sfermion mass terms as interactions, we
perform a perturbative expansion of FCNC amplitudes in terms of mass insertions.
The lowest non-vanishing order of this expansion gives an excellent 
approximation to the full result, given the tight experimental constraints 
on flavour-changing
mass insertions. It is most convenient to work in the super-CKM basis, in which
all gauge interactions carry the same flavour dependence as in the SM. In this
basis, we define the mass insertions $(\delta^d_{ij})_{AB}$ as the off-diagonal
mass terms connecting down-type squarks of flavour $i$ and $j$ and helicity $A$
and $B$, divided by the average squark mass (see sec. \ref{sec:susy}).

The constraints on $(\delta^d_{23})_{AB}$ have been studied in detail in
ref.~\cite{Ciuchini:2006dx} using as experimental input the branching ratios
and CP asymmetries of $b \to s \gamma$ and $b \to s \ell^+ \ell^-$ decays and
the first measurement of $B_s - \bar B_s$ mixing. We perform the same analysis
using the full information encoded in $C_{B_s}$ and $\phi_{B_s}$, and the
recently computed NLO corrections to the $\Delta B=2$ SUSY effective
Hamiltonian~\cite{Ciuchini:2006dw}. We refer the reader to ref.~\cite{vale} for
all the details of this analysis.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[p]
\begin{center}
\includegraphics[width=0.45\textwidth]{mixing/PLOTS/d_ll_all350} 
\includegraphics[width=0.45\textwidth]{mixing/PLOTS/d_rr_all350} \\
\includegraphics[width=0.45\textwidth]{mixing/PLOTS/d_lr_all350} 
\includegraphics[width=0.45\textwidth]{mixing/PLOTS/d_rl_all350} \\
\includegraphics[width=0.45\textwidth]{mixing/PLOTS/d_llrr_all350}
\caption{Allowed range in the
Re$\left(\delta^d_{23}\right)_{AB}$-Im$\left(\delta^d_{23}\right)_{AB}$ plane,
with $AB=LL$ (top left), $AB=RR$ (top right), $AB=LR$ (middle left), $AB=RL$
(middle right) and $AB=LL$ with $\left(\delta^d_{23}\right)_{LL} =
\left(\delta^d_{23}\right)_{RR}$ (bottom).}
\label{fig:susy}
\end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For definiteness, we present here the results obtained by choosing an average
squark mass of $350$ GeV, a gluino mass of $350$ GeV, $\mu=-350$ GeV and $\tan
\beta=3$. The dependence on $\mu$ and on $\tan \beta$ is induced by the
presence of a chirality flipping, flavour conserving mass insertion 
proportional
to $\mu\tan \beta$. In Fig.~\ref{fig:susy}, we show the allowed ranges in the
Re$\left(\delta^d_{23}\right)_{AB}$-Im$\left(\delta^d_{23}\right)_{AB}$ planes.
The corresponding upper bounds at 95\% probability are presented in
Table~\ref{tab:susy}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\begin{center}
\caption{Upper bounds at 95\%  probability on the mass insertion parameters
$\vert\left(\delta^d_{23}\right)_{AB}\vert$, see the text for details.}
\label{tab:susy}
\begin{tabular}{|c|c|c|c|}
\hline
$ \left\vert\left(\delta^d_{23}\right)_{LL}\right\vert$ &
$ \left\vert\left(\delta^d_{23}\right)_{RR}\right\vert$ &
$ \left\vert\left(\delta^d_{23}\right)_{LL=RR}\right\vert$ &
$ \left\vert\left(\delta^d_{23}\right)_{LR,RL}\right\vert$ \\ 
\hline {\phantom{\huge{l}}}
$2\cdot 10^{-1}$ & $7 \cdot 10^{-1}$ & $5\cdot 10^{-2}$ & $5 \cdot 10^{-3}$\\
\hline
\end{tabular}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

One finds that the constraints on $\left(\delta^d_{23}\right)_{LL}$ and
$\left(\delta^d_{23}\right)_{LL}= \left(\delta^d_{23}\right)_{RR}$ come from the
interplay of $B_s - \bar B_s$ mixing with $b\to s$ decays.
$\left(\delta^d_{23}\right)_{RR}$ is dominated by the information on $B_s - \bar
B_s$ mixing, while $\left(\delta^d_{23}\right)_{LR}$ and
$\left(\delta^d_{23}\right)_{RL}$ are dominated by $\Delta B=1$ processes.

\subsubsection{$B_s - \bar B_s$ in SUSY with minimal flavour violation}

As a second model-specific case for meson mixing we mention that of SUSY with
Minimal Flavour Violation (MFV). The MFV scenario is defined, in general, 
within
the effective field theory approach of ref.~\cite{D'Ambrosio:2002ex}. In the
specific case of SUSY, the soft squark mass terms, parametrised in the previous
section in terms of mass insertions, are expanded in terms of the SM Yukawa
couplings \cite{D'Ambrosio:2002ex,Hall:1990ac} and the relevant parameters
become the expansion coefficients. A detailed meson mixing study within this
approach has been performed in ref.~ \cite{Altmannshofer:2007cs} and for low
$\tan \beta$ shows that: (i) NP contributions are {\em naturally} small, for
$\Delta M_s$ of the order of $1/$ps; (ii) such contributions are always
positive; (iii) if $\mu$ is not small, gluino contributions enhance (even for
low $\tan \beta$) scalar operators, which then spoil the phenomenological
picture of (V-A)$\times$(V-A) dominated MFV \cite{Buras:2000dm}. In particular
item (i) emphasises the importance of precision determinations for lattice
parameters like $\xi$, if NP is of minimal flavour violating nature.




\subsubsection{Present experimental situation}
\label{sec:EXP}

New information concerning the \Bs mixing parameters became available 
during the workshop
{\it Flavour in the Era of the LHC}. The highlight was the measurement
of \dms by D\O\ and CDF. The D\O\ experiment used the semileptonic \bsmunux
decays with \dsphipi, and determined a 90\% confidence range for \dms : $ 17 <
\Delta m_s < 21\ {\rm ps}^{-1} $. The initial CDF result yielded a 3$\sigma$
observation of \bsmix mixing by making use of semileptonic and hadronic decay
modes \cite{Abulencia:2006mq}. Shortly after CDF published an improved analysis
\cite{Abulencia:2006ze}. In this analysis the signal yield was increased by
improving the particle identification and by using a neural network for the
event selection, which allows the use of additional decay modes. Moreover the
flavour tagging was improved by adding an opposite-side flavour tag based 
on the
charge of the kaons, and by the use of a neural network for the combination of
the kaon, lepton and jet-charge tags. The result for \dms equals 
\begin{equation}\label{bsmixexp}
\Delta m_s = 17.77 \pm 0.010 \pm 0.07\ {\rm ps}^{-1}. 
\end{equation}
The probability that a statistical fluctuation would
produce this signal is $8 \times 10^{-8}$ ($> 5\sigma$ evidence). 
This value for \dms is consistent with the SM expectation, 
see eq.~(\ref{eq:dms-sm}). The ratio
$|V_{td}/V_{ts}|$ was determined by CDF as well \cite{Abulencia:2006ze}, and
equals $0.2060 \pm 0.0007 (\dms) \apm{0.0081}{0.0060} (\dmd + {\rm theory})$.

Also information on the \Bs mixing phase became available \cite{Abazov:2007tx}. 
The D\O\ experiment performed two independent measurements of 
$A^{s}_{SL}$, defined in (\ref{eq:A_SL_s}), using
the same sign di\-muon pairs~\cite{Abazov:2006qw} and time-integrated
semileptonic decays $B_{s} \to \mu\nu D_{s}$ with $D_{s} \to
\phi\pi$~\cite{Abazov:2007nw}.

The same sign dimuon asymmetry in $B$ decays at Tevatron can be expressed
as~\cite{Grossman:2006ce}:
\begin{eqnarray}
A_{SL} & = & \frac{N(b\bar{b}\to \mu^{+} \mu^{+} X) - 
N(b\bar{b} \to \mu^{-} \mu^{-} X)}{N(b\bar{b}
\to \mu^{+} \mu^{+} X) + N(b\bar{b} \to \mu^{-} \mu^{-} X} 
= \frac{f_{d}Z_{d}A^{d}_{SL}+f_{s}Z_{s}A^{s}_{SL}}{f_{d}Z_{d}+f_{s}Z_{s}},
\label{eq:A_SL} \\
Z_{q} & = & \frac{1}{1-y^{2}_{q}} - \frac{1}{1+x^{2}_{q}}\ , \qquad
x_{q} = \Delta M_{q} / \Gamma_{q}\ , \qquad  y_{q} = \Delta\Gamma_{q}/
(2\Gamma_{q}). \nonumber
\end{eqnarray}
Here $f_{d} = 0.398\pm 0.012$ and $f_{s} = 0.103 \pm 0.014$ are the  \Bd  and
\Bs fragmentation fractions. The measured asymmetry $A_{SL}$ was presented by
D\O\  in Ref.~\cite{Abazov:2006qw}:
\begin{equation}
A_{SL}(\mathrm{D\O} )= A^{d}_{SL}+\frac{f_{s}Z_{s}}{f_{d}Z_{d}}A_{SL}^{s}
=-0.0092\pm 0.0044(stat.)\pm 0.0032(syst.).
\label{eq:A_SL_D0_1}
\end{equation}
Measurements of $A_{SL}^{d}$ were performed by the $b$ factories. The average
value of $A_{SL}^{d}$ is~\cite{Grossman:2006ce}:\\ 
%
\begin{equation}
 A_{SL}^{d} = +0.0011 \pm 0.0055\; .   
\end{equation}
%
This leads to the value of $A_{SL}^{s}$ from the same sign dimuon
asymmetry: 
%
\begin{equation}
 A_{SL}^{s} = -0.0064 \pm 0.0101 \;. 
\end{equation}
%
Recently D\O\ has also presented a time-integrated direct measurement of $A{SL}^{s}$  
using semileptonic $B_s \to D^{\pm}\mu^{\mp}\nu_{\mu}$ decays~\cite{Abazov:2007nw}.
They measure:
%
\begin{equation}
A_{SL}^{s} = +0.0245\pm 0.0193(stat.) \pm 0.0035(syst.).
\label{eq:A_SL_S_2}
\end{equation}
%
%
These two measurements of $A_{SL}^{s}$ are independent and their combination
gives the charge asymmetry in semileptonic \Bs decays: 
$ A_{SL}^{s} = 0.0001 \pm 0.0090$~\cite{Abazov:2007zj}.
The analysis of the time-dependent angular distributions in  
$B_{s}\to J/\psi \phi$ decays yields both the decay width difference
$\Delta\Gamma_{s}$ and CP violating phase $\phi_{s}$~\cite{Abazov:2007tx}:
%
\begin{eqnarray}
\Delta\Gamma_{s} & = 0.17 \pm 0.09 \pm 0.03~\mathrm{ps}^{-1} \; , \nonumber\\
\phi_{s}  & =- 0.79\pm 0.56 \pm 0.01\;.
\end{eqnarray}
%
 Combining the results for $ A_{SL}^{s}$,
$\Delta\Gamma_{s}$, $\phi_{s}$ and using the CDF result on the mass difference
\dms~\cite{Abulencia:2006ze} gives an improved estimate for $\phi_{s}$ and
$\Delta\Gamma_{s}$~\cite{Abazov:2007zj}:
: 
%
\begin{eqnarray}
\Delta\Gamma_{s} & = 0.13 \pm 0.09 ~\mathrm{ps}^{-1} \; , \nonumber\\
\phi_{s}  & =- 0.70^{+0.47}_{-0.39}\;. 
\end{eqnarray}
%
Also new results have been released recently concerning the \Bs lifetime and
\dg. At D\O\ the \Bs lifetime for \bsmunux was measured to be $1.398 \pm
0.044(stat) \apm{0.028}{0.025} (sys)$ ps$^{-1}$~\cite{Abazov:2006cb}. The
average \Bs lifetime equals $1.466 \pm 0.059$ ps$^{-1}$~\cite{Yao:2006px}. 
CDF published the measurement of 
$\dg=0.47\apm{0.19}{0.24} (stat) \pm 0.01 (sys)\, {\rm ps}^{-1}$ 
\cite{Acosta:2004gt}.

%\subsubsection{Experimental outlook : LHC}

In the near future the LHC experiments LHCb, ATLAS and CMS
will start to provide information on \bsmix mixing. 
In the following sections the sensitivity of LHCb  
to the \Bs mixing parameters \dms, \dg, \phis and \asl 
and the prospects for CMS will be discussed.

\subsubsection{LHCb}

The LHCb experiment is designed as a single-arm forward spectrometer to study
$b$ decays and CP violation. Its main characteristics are precise vertexing,
efficient tracking and good particle identification. The high-precision
measurements at LHCb will enable further tests of the CKM picture, and probe
physics beyond the SM. This is in particular true for the measurement of \bsmix
mixing parameters such as \dms, \dg, $\Pphi_\Ps$ and \asl.

LHCb will run at a nominal luminosity of  ${\mathcal L} =
2\times10^{32}\:\text{cm}^{-2}\text{s}^{-1}$. Assuming a $b\bar b$ production
cross-section of $\sigma_{\Pb\Pab} = 500\:\mu\text{b}$, this will correspond to
an integrated luminosity of $2\:\text{fb}^{-1}$ per nominal year of
$10^7\:\text{s}$ of data taking. All event yields quoted below are for
$2\:\text{fb}^{-1}$. They have been obtained from a full Monte Carlo (MC)
simulation of the experiment, which included the following: pileup generation,
particle tracking through the detector material, detailed detector response
(including timing effects such as spillover), full trigger simulation, offline
reconstruction with full pattern recognition, and selection cuts.
High-statistics samples of signal events have been produced for a detailed 
study of resolutions and efficiencies. Combinatorial background has been 
studied using
a sample of $\sim 27$M inclusive $b\bar b$ events corresponding to about 10
minutes of data taking, while identified physics background sources have been
studied with large specific background samples.

\subsubsubsection{Sensitivity to \dms from \bsdspi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
\begin{center}
%\epsfig{file=mixing/PLOTS/massBs_BsDsPi.eps,width=0.48\textwidth} \hfill
%\epsfig{file=mixing/PLOTS/tau_cuts_tag_HLT.eps,width=0.48\textwidth}
\includegraphics[width=0.48\textwidth]{mixing/PLOTS/massBs_BsDsPi.eps} \hfill
\includegraphics[width=0.48\textwidth]{mixing/PLOTS/tau_cuts_tag_HLT.eps}
\caption{\underline{Left}: Reconstructed \bsdspi mass distribution from full MC
simulation, after trigger and all selection cuts~\cite{bib:LHCb-2007-xxx_Borel}.
The points with error bars represent the signal (on an arbitrary vertical scale).
The histogram represents the $B\to D^-\pi^+$ background and the dotted flat
line represents the upper limit of the combinatorial background from $b\bar b$
events, normalised to the signal.
\underline{Right}: Reconstructed \bsdspi proper time distribution from full MC
simulation of the signal, corresponding to an integrated luminosity of
$0.5\:\text{fb}^{-1}$~\cite{bib:LHCb-2007-xxx_Borel}. The lower histogram
represents the events tagged as mixed. The background is not shown.}
\label{fig:LHCb/BsDspi_mass}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The mass difference \dms between the mass eigenstates of the \bsmix system is
best measured as the frequency of the oscillatory behaviour of the proper time
distribution of flavour-tagged \PBs mesons decaying to a flavour-specific final
state. The best channel for this at LHCb is \BsDspi, with the subsequent 
$D^+_s$ decay to $K^+K^-\pi^+$, because of its easy topology with four 
charged tracks and its relatively large branching fraction of 
% (3.4 +-0.7)*1e-3*(5.2 +-0.9)*1e-2 = (1.77 +-0.48)*1.e-4
$B(\BsDspi)\times B(D^+_s\to K^+K^-\pi^+) = (1.77 \pm 0.48)\times
10^{-4}$~\cite{bib:LHCb-2007-xxx_Borel}. 
Such decays can be detected, triggered,
reconstructed and selected with a final mass resolution of $\sim 14$~MeV$/c^2$
(see Fig.~\ref{fig:LHCb/BsDspi_mass} left) and a total efficiency of about
0.4\%, leading to a yield of $\rm (140k \pm 40k)$ events in $2\:\text{fb}^{-1}$.
After the trigger and selection, the combinatorial background is expected to be
dominated by $b\bar b$ events, and has been estimated to be less than 5\% of the
signal at 90\% CL, in a $\pm 50$~MeV/$c^2$ mass window around the signal. Using
the same sample of simulated $b\bar b$ events, the background from partially
reconstructed $b$-hadron decays in the same mass window has been estimated 
to be less than 40\% at 90\% CL. 
This includes partially reconstructed $\Lambda_b$
and $B_d$ decays. A dedicated study showed that the background from
$B\to D^-\pi^+$ decays (where one of the charged pions from the $D$ decay
could be misidentified as a kaon) is approximately 5\% of the signal.

The proper time resolution, obtained on an event-by-event basis from the
estimated tracking errors, typically varies between 15~fs and 80~fs with an
average value of $\sim 40$~fs (dedicated studies are being done at LHCb to 
model the proper time resolution~\cite{LHCb_Peter} and to verify the 
estimated tracking errors~\cite{LHCb_Stefania} with data).
% 33 fs (average estimated error) * 1.175 (pull)
A flavour tagging power of $\epsilon D^2$ of at least 9\% 
is achieved on the MC signal, 
% 0.63*(1-2.*0.31)**2 according to Luis
combining several tags in a neural network: a muon or electron from the
$b\to\ell$ decay of the other $b$-hadron, a charged kaon from the
$b\to c\to s$ decay of the other $b$-hadron, the vertex charge of the other
$b$-hadron, and a charged kaon accompanying the signal $B_s$ in the 
fragmentation chain~\cite{bib:lhcb-2007-058}.

The statistical uncertainty on the measurement of \dms using an integrated
%luminosity of $0.5\:\text{fb}^{-1}$ (first year of data-taking) is expected to
%be $\pm 0.006$~ps$^{-1}$. 
luminosity of $2\:\text{fb}^{-1}$  is expected to
be $\pm 0.007$~ps$^{-1}$~\cite{DSKRECSENS}. 
It will be dominated by systematic uncertainties
related to the determination of the proper time scale.
Figure~\ref{fig:LHCb/BsDspi_mass} (right) shows the proper time distribution
from which such a measurement could be extracted. 

The \BsDspi sample will play a crucial role as a control sample in all
time-dependent \PsB analyses; indeed it can be used to measure directly the
dilution (due to flavour tagging and proper time resolution) on the $\sin(\dms
t)$ and $\cos(\dms t)$ terms in time-dependent CP asymmetries. It will also be
used as a normalisation channel for many measurements of $B_s$ branching 
fractions.
More details on the selection of  \BsDspi events can be found in 
Ref.~\cite{bib:LHCb-2007-xxx_Borel}.

\subsubsubsection{Sensitivity to \phis and \dg from exclusive \bccs decays}

The \bsmix mixing phase $\phi_s$ can be measured from the
flavour-tagged \Bs decays to CP eigenstates involving the \bccs quark-level
transition. The best mode for this at LHCb is \Bsjpphi. However, in this case,
the vector nature of the two particles in the final state causes their relative
angular momentum to take more than one value, resulting in a mixture of CP-even
and CP-odd contributions. An angular analysis is therefore required to separate
them on a statistical basis. This can be achieved with a simultaneous fit to the
measured proper time and so-called transversity angle of the reconstructed
decays. Such a fit is sensitive also to \dg because of the presence of the two
CP components.

The sensitivity to $\phi_s$ has been studied so far with the following modes:
\begin{itemize}
\item
$B_s\to J/\psi(\mu^+\mu^-)\phi(K^+K^-)$~\cite{bib:Fernandez_thesis,
bib:LHCb-2006-047_LF}
\item $B_s\to\eta_c(\pi^+\pi^-\pi^+\pi^-, \pi^+\pi^- K^+K^-,
K^+K^-K^+K^-)\phi(K^+K^-)$~\cite{bib:Fernandez_thesis,
bib:LHCb-2006-047_LF}
\item $B_s\to J/\psi(\mu^+\mu^-)\eta(\gamma\gamma,
\pi^+\pi^-\pi^0)$~\cite{bib:Fernandez_thesis,bib:LHCb-2006-047_LF}
\item $B_s\to J/\psi(\mu^+\mu^-)\eta'(\eta(\gamma\gamma)\pi^+\pi^-,
 \rho(\pi^+\pi^-)\gamma)$~\cite{bib:LHCb-2007-xxx_DV,bib:LHCb-2007-xxx_SJO}
\item
$B_s\to D^+_s(K^+K^-\pi^+)D^-_s(K^+K^-\pi^-)$~\cite{bib:Fernandez_thesis,
bib:LHCb-2006-047_LF}
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tbp]
\begin{center}
\caption{Characteristics of different exclusive \bccs modes for the measurement
of $\phi_s$. The first 6 columns of numbers are obtained from the full MC
simulation. They represent the expected number of triggered, reconstructed and
selected signal events with an integrated luminosity of 2\:$\text{fb}^{-1}$
(before tagging), the background-over-signal ratio determined mainly from
inclusive $b\bar b$ events, the \Bs mass resolution, the average value of the
estimated event-by-event \Bs proper time error scaled by the width of its pull
distribution, the flavour tagging efficiency, and the mistag probability. These
parameters have been used as input to a fast MC simulation to obtain the
sensitivity on $\phi_s$ given in the last column. The last line describes the
control channel (see text).}
\begin{tabular}{|l|r|l|c|c|c|c|c|}
\hline
Channel &  2\:$\text{fb}^{-1}$ & $B/S$ & 
$\sigma_{\rm mass}$ & $\sigma_{\rm time}$ & 
$\epsilon_{\text{tag}}$ & $\omega_{\text{tag}}$ & $\sigma(\phi_s)$ \\
& yield && [~\MeVctwo~] & [~fs~] &   [~\%~] & [~\%~] & [~rad~]  \\
\hline
\Bsjpphi          & 131k & 0.12 & 14 & 36 & 57 & 33 & 0.023 \\
\Bsetacphi        &   3k & 0.6  & 12 & 30 & 66 & 31 & 0.108 \\
\Bsjpetagg        & 8.5k & 2.0  & 34 & 37 & 63 & 35 & 0.109 \\
\Bsjpetappp       & 3k   & 3.0  & 20 & 34 & 62 & 30 & 0.142 \\
\Bsjpetaprimetapp & 2.2k & 1.0  & 19 & 34 & 64 & 31 & 0.154 \\
\Bsjpetaprimrhog  & 4.2k & 0.4  & 14 & 29 & 64 & 31 & 0.080 \\
\BsDsDs           & 4k   & 0.3  &  6 & 56 & 57 & 34 & 0.133 \\
\BsDspi           & 140k & 0.4  & 14 & 40 & 63 & 31 & ---   \\
\hline
\end{tabular}
\label{tab:LHCb_phis}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.80\textwidth]{mixing/PLOTS/TauBsErr_All.eps} \hfill
%\epsfig{file=LHCb/TauBsErr_All.eps,width=0.68\textwidth}
\end{tabular}
\caption{Distribution of the event-by-event proper time resolution [fs]
for different $B_s$ channels, as obtained
from the full MC simulation. The normalisation is arbitrary.}
\label{fig:sensitivity/TauBsErr_All}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The results are summarised in Table~\ref{tab:LHCb_phis}. For each signal event
in the full simulation the proper time and its error are estimated using a
least-squares fit. The distributions of the proper time errors (scaled with the
sigma of their pull distribution) are shown in
Fig.~\ref{fig:sensitivity/TauBsErr_All}. Most channels have a proper time
resolution below 40\:fs. A good proper time resolution is important 
for resolving the fast \bsmix oscillations.

The sensitivities to the \bsmix mixing parameters are determined by means
of fast parameterised simulations, 
with the results of Table~\ref{tab:LHCb_phis}
as inputs. A large number of experiments are generated assuming the following
set of parameters: $\Delta m_s = 17.5\ \text{ps}^{-1}$, $\phi_s =
-0.04\ \text{rad}$, $\Delta \Gamma_\Ps/\Gamma_{\Ps} = 0.15$, $1/\Gamma_{\Ps} =
1.45\ \text{ps}$, and a fraction of CP-odd component of $R_T = 0.2$ (for
\Bsjpphi). The different parameters are extracted by performing a 
likelihood fit
to the mass, proper time, and transversity angle (for \Bsjpphi) distributions,
including a background contribution. The \bccs likelihood is simultaneously
maximised with a similar likelihood for the \BsDspi control sample such as to
constrain \dms and the mistag fraction from the data. The background properties
are determined from the $B_s$ mass sidebands. The physics parameters, extracted
in the signal region with all other parameters fixed, are \phis, \dms,
$\Delta \Gamma_\Ps/\Gamma_{\Ps}$, $1/\Gamma_\Ps$, $\omega_{\text{tag}}$, and
$R_{T}$ (for \Bsjpphi).

The sensitivities to \phis for the different channels, obtained as the rms
of the distribution of the fit results, are given in the last column of
Table~\ref{tab:LHCb_phis}. They gently decrease with increasing $|\phi_s|$,
and do not depend much on $\Delta \Gamma_\Ps/\Gamma_{\Ps}$. For instance, the
statistical uncertainty on \phis for $\phi_s = -0.2\:\text{rad}$ is
$\pm 0.026\:\text{rad}$ from \Bsjpphi alone, with
$2\:\text{fb}^{-1}$~\cite{bib:Fernandez_thesis}. The best performance is
achieved with the \Bsjpphi sample, which also yields a statistical precision of
$\pm 0.0092$ on $\Delta \Gamma_\Ps/\Gamma_{\Ps}$ (2\:$\text{fb}^{-1}$). The
$\phi_s$ sensitivities obtained from the other modes (which are pure
CP-eigenstates) are not as good, but still interesting. Combining all modes, a
statistical uncertainty $\sigma(\phi_s) = \pm 0.0092\:\text{rad}$ is 
expected after $10\:\text{fb}^{-1}$.

LHCb has the potential to perform the first significant measurement of 
$\phi_s$, test the consistency with the SM expectations, and possibly
uncover New Physics that may be hiding in \bsmix mixing.


\subsubsubsection{Sensitivity to $A^{s}_{SL}$ from \bsmunux and \bsdspi }

The CP-violating charge asymmetry $A^{s}_{SL}$ is an important parameter 
to constrain new physics contributions in $B_s$ mixing, 
see Section~\ref{sec:NP}. 
$A^s_{SL}$ 
is accessible by measuring the charge 
asymmetry of the time-integrated rates of untagged $B_s$ 
decays to flavour-specific final 
states such as $D_s^- \mu^+ \nu X$ or $D_s^-\pi^+$~\cite{Nierste:2004uz}. 
In LHCb the asymmetry $A^s_{SL}$ is measured by  
fitting the time-dependent decay rates.
This method allows a determination of $A^s_{SL}$ also 
for a non-zero production asymmetry of 
$B_s$ and $\bar {B}_s$ mesons
which, at the LHC, is expected to be of ${\cal O}(1\%)$. 
Based on a large sample of fully 
simulated inclusive $b\bar{b}$ events and a dedicated signal sample, 
LHCb estimates 
a signal yield of 1M \bsmunux events in $2\:\text{fb}^{-1}$ of data, 
with a $B/S$ ratio of about 0.36~\cite{Xie1}. 
This leads to a statistical precision of 
$\pm 0.002$ on $A^s_{SL}$~\cite{Xie2}.
A similar analysis based on 140k \bsdspi events is expected 
to reach a precision of $\pm 0.005$ with the 
same integrated luminosity of $2\:\text{fb}^{-1}$~\cite{Xie2}. 
Systematic uncertainties are 
expected to be dominated by the detector charge asymmetry, 
which needs to be 
determined separately. 
A method is proposed to control the  detector charge asymmetry
by measuring the 
difference $A^s_{SL}-A^d_{SL}$ using \Bs and \Bd decays to the same final state, e.g. 
 $\Bs \rightarrow D_s^-\mu^+\nu X$ and $\Bd \rightarrow D^-\mu^+\nu X$, where 
$D_s^- \rightarrow K^+K^-\pi^-$ and $D^- \rightarrow K^+K^-\pi^-$.


\subsubsubsection{Correcting for trigger biases in lifetime fitting at LHCb}

Lifetime measurements at LHCb will help for the detector calibration and 
provide tests of theoretical predictions based on the heavy-quark expansion. 
In order to exploit the full range of decays available at LHCb, it is 
important to have a
method for fitting lifetimes in hadronic channels, which are biased by the
impact parameter cuts in the trigger. We have investigated a Monte-Carlo
independent method to take into account the trigger effects. 
The method is based
on calculating event-by-event acceptance functions from the decay geometry and
does not require any external input. Current results with the method are given
in ~\cite{vava-lhcb1}. The method is described, for the case of two-body 
decays, in~\cite{Rademacker:2005ay}.

The decay $B_{d} \to D^{-} \pi^{+}$ has an expected yield of 1.34M 
events per $2\:\text{fb}^{-1}$. 
The $S/B$ ratio is expected to be around 5~\cite{DPIREC}.
Fitting the $B_d$ lifetime with 60k toy Monte Carlo signal events achieves a
statistical precision of 0.007~ps, while fitting to 60k signal and 15k 
background
events achieves a precision of 0.009~ps (the current world average is 1.530 $\pm$
0.009 ps \cite{Yao:2006px}). A similar result is seen in data generated with the
full LHCb detector simulation~\cite{vava-lhcb1}. Therefore, although the
systematic errors associated with this method are unknown at the moment, we can
expect a very good measurement of the \Bd lifetime using the decay
$B_{d}\to D^{-} \pi^{+}$.


%\subsubsubsection{ATLAS: Sensitivity to $\phi_s$ and \dg}

\subsubsection{CMS}

\subsubsubsection{Sensitivity to \dg}

Also at CMS the decay
$B_s \to J/\psi \, \phi \to \mu^+\mu^- K^+K^-$ 
is being studied~\cite{CMS_NOTE_2006-090}. Several important
background processes have been identified. The prompt \jpsi production is the
main source of background at trigger level, since it represents a dominant
contribution to the Level-1 dimuon trigger rate. For the off\-line selection, 
the main background is the inclusive decay $b\to\jpsi\, X$. 
The decay $B_d \to J/\psi \, K^{*0}\to \mu^+\mu^- K^+ \pi^-$ 
is of particular concern,
since the pion can be mistaken to be a kaon, and hence the decay be
misidentified as \bspsiphi\ . Furthermore, the final state of
this \Bd decay also displays a time-dependent angular distribution similar to
that of the \Bs decay under study, 
with different physical parameters. The \Bs decay
chain is selected at Level-1 by the dimuon trigger. 
The latter demands two muons
with a transverse momentum above $3\GeVc$, and the additional requirement that
these muons have opposite charge can be used.

In the HLT~\cite{DAQTDR}, $b$ candidates are identified by doing a partial
reconstruction of the decay products in the tracker in restricted tracking
regions and imposing invariant mass and vertex requirements~\cite{PTDR1}.

The HLT selection of the decay \bspsiphi\ has been separated in two steps. In
the first, called Level~2, \jpsi candidates with a displaced vertex are
identified. Tracks are then reconstructed in the tracking regions defined 
by the
Level~1 muon candidates, and all track pairs of opposite charge for which the
invariant mass is within $150\MeVcc$ of the world-average \jpsi mass are
retained. To remove the prompt \jpsi background, the two muon candidates are
then fitted to a common decay vertex and the significance of the transverse
decay length is required to be above $3$. With this selection, 
the accepted rate is reduced to approximately 15~Hz, with 80\% of the 
\jpsi originating in the decay of $b$ hadrons.

Next, at Level~3, a further reduction is achieved by doing a full
reconstruction of the \Bs decay. To reconstruct the kaons, the tracking region
is chosen around the direction of each \jpsi candidate. Assigning the kaon mass
to the reconstructed tracks, all oppositely charged track pairs for which the
invariant mass is within $20\MeVcc$ of the world-average mass of the $\phi$
meson are retained, for a resolution in the invariant mass of the $\phi$ meson
of $4.5\MeVcc$. With the two muon candidates, the four-track invariant mass is
required to be within $200\MeVcc$ of the world-average mass of the \Bs meson.
The resolution in the invariant mass of the \Bs meson is found to 
be $65\MeVcc$.
Here as well, a vertex fit of the four tracks is performed, imposing a similar
requirement as above. The total rate for this selection is well below 0.1~Hz,
and a yield of approximately $456000$ signal events can be expected within
$30\fbinv$ of data.

In the offline selection, candidates are reconstructed by combining two muons of
opposite charge with two further tracks of opposite charge. As CMS does not
possess a particle identification system suitable for this measurement, all
measured tracks have to be considered as possible kaon candidates, which adds a
substantial combinatorial background. A kinematic fit is made, where the four
tracks are constrained to come from a common vertex and the invariant mass of
the two muons is constrained to be equal to the mass of the \jpsi. With this
fit, a resolution on the invariant mass of the \Bs meson of $14\MeVcc$ is found.
The invariant mass of the two kaons is required to be within $8\MeVcc$ of the
world-average mass of the $\phi$ meson.

With this selection, a yield of approximately 327\,000 signal events can be
expected within $30\fbinv$ of data, with a background of 39\,000 events. These
do not include a requirement on the four-track invariant mass of the candidates,
since the sidebands could be used later in the analysis. However, only a small
fraction of these events are directly under the \Bs peak, and even a simple cut
will reduce the number of background events by a significant factor.

\providecommand{\apar}{\ensuremath{A_{\parallel}}}
\providecommand{\aperp}{\ensuremath{A_{\perp}}}
\providecommand{\azero}{\ensuremath{A_{0}}}
\providecommand{\gh}{\ensuremath{\Gamma_H}}
\providecommand{\gl}{\ensuremath{\Gamma_L}}

\providecommand{\psinv} {\mbox{\ensuremath{\mathrm{\; ps}^{-1}}}}
\providecommand{\pdl} {proper decay length}
\providecommand{\pdf}{p.d.f.}

The measurement of the width difference {\dg} can now be done on this sample of
untagged \Bs candidates. As mentioned earlier, the $J/ \psi\, \phi$ final state 
is an admixture of CP-even and CP-odd states, and an angular analysis is
required~\cite{Dunietz:2000cr}. As the CP-even and CP-odd components have
different angular dependences and different time evolutions, the different
parameters can be measured by performing an unbinned maximum likelihood fit on
the observed time evolution of the angular distribution. In the absence of
background and without distortion, the \pdf\ describing the data would be the
original differential decay rate. The distortion of this distribution by the
detector acceptance, trigger efficiency and the different selection criteria
must be taken into account by an efficiency function modelling the effect of 
the decay length requirements and the distortion of the angular distribution.

A sample corresponding to an integrated luminosity of $1.3\fbinv$ 
was considered, which allows us to have a realistic ratio of misidentified 
$B_d\to J/\psi\, K^*$ and signal events. 
With the low number of background events that remain after all
selection requirements, an accurate modelling of the background is not 
possible, neither of its angular distribution
nor of its time-dependent efficiency. Therefore the background events
are simply added to the data set and their expected distribution is not included
in the \pdf\ used in the fit. The \pdf\ then simply describes the \Bs
distribution. With such a fit, in which the invariant mass of the candidates is
not taken into account, a restriction on the invariant mass of the candidates
should obviously be made. Choosing a window of $\pm 36\MeVcc$ around the
world-average \Bs mass reduces the number of \Bd background events by another
59\%, while reducing the number of signal candidates by only 2.9\%. The
result of the fit is given in Table~\ref{tab:final}, where both the statistical
and expected systematic uncertainties are quoted. A first measurement of the
width difference of the weak eigenstates could thus be made with an
uncertainty of 20\%. On a larger sample, corresponding to an integrated
luminosity of $10\fbinv$, it is foreseen that the statistical uncertainty 
would be reduced to 0.011.

\begin{table*}[!tbh]
\caption{Results of the maximum likelihood fit for an integrated
luminosity of $1.3\fbinv$ (signal and background).}
\label{tab:final}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Parameter	&Input value  & Result  & Stat. error & Sys. error & Total error
&  Rel. error \\
\hline
$|A_0(0)|^2$	& 0.57        &  0.5823   & 0.0061  &0.0152& 0.0163& 2.8\%\\
$|A_{||}(0)|^2$	& 0.217       &  0.2130   & 0.0077  &0.0063&0.0099& 4.6\%\\
$|A_\bot(0)|^2$	& 0.213       &  0.2047   &  0.0065&0.0099& 0.0118& 5.8\%\\
\gm		& 0.712\psinv & {0.7060}\psinv   & {0.0080}\psinv & 0.0227\psinv
& 0.0240\psinv &3.4\% \\
\dg		& 0.142\psinv & {0.1437 }\psinv  &{0.0255} \psinv & 0.0113\psinv
& 0.0279\psinv &19\% \\
\dgg		& 0.2         & 0.2036  & 0.0374 & 0.0173&0.0412&20\%\\
\hline
\end{tabular}
\end{center}
\end{table*}

\subsubsubsection{Missing particles in the reconstruction}

The best way to study the \bsmix oscillations is to have a fully
reconstructed final state of the \Bs decay. The disadvantage of such decay
channels is the limited statistics. Much more signal events can be 
collected in semileptonic decays as $\Bs \to \Dsm \ellp \nu$. 
Due to the missing
neutrino in this decay the \Bs momentum, and hence the proper-time resolution
for the \Bs, is less precise than in the fully reconstructed case, even if a
correction ($k$-factor) is applied.  
However, recently a new method ($\nu$-reco)
has been proposed \cite{Dambach:2006ha}, which allows us to calculate 
the neutrino momentum with the help of vertex information.

In order to verify the $\nu$-reco method a MC simulation has been 
developed to study \bsmix mixing in the semileptonic decay mode. 
Kinematical cuts, track parameters
and vertex positions (primary and secondary) have been simulated according to
typical hadron collider detector
conditions~\cite{Abe:1998cj,Abazov:2006cb,Starodumov:1997,atlas:1999fq}. 
The proper time resolution obtained is $\sigma = 132\fs$
with the $k$-factor method and $\sigma = 91\fs$ with the $\nu$-reco method. 



==> neutrinos/neutrinomode_exp.tex <==
\subsection{Experimental Prospect for neutrino modes}
%We discuss experimental prospect for measurements of the neutrino modes.

\subsubsection{Overview}
%We explain in this subection,
%\begin{itemize}
%\item Advantage of $e^+e^-$ $B$-factory, and necessity of super $B$-factory
%to measure the neutrino modes.
%\item General feature of the analysis using fully reconstructed tag. 
%\item Assumption in the studies described in the following subsections;
%integrated luminosity (5/50 ab$^{-1}$), tagging efficiency and quality
%(we basically assume the same performance). 
%\item Others
%\end{itemize}

Experimental prospects for neutrino modes, such as $B \to X_s\,\nu\,\bar\nu$, 
$B \to \tau\,\bar\nu$ and $B \to X_c\,\tau\,\bar\nu$, are discussed.
Because of the missing multiple neutrinos in the final state, these
decays lack kinematic constraints, which can be used to surpress 
background processes.
The $e^+e^-$ $B$-factories, where background is relatively low and can
be reduced by reconstructing the accompanying $B$ meson, would be the 
ideal place to measure these decays.
We also discuss the prospect for $B \to \mu\,\bar\nu$, which can be
used to test the lepton universality in comparison to $B \to \tau \nu$.

Belle and BaBar have used hadronic decays to reconstruct the
accompanying $B$ (hadronic tags), for which the tagging efficiency
is about 0.3(0.1)\% for the charged (neutral) $B$ meson.
BaBar has used also semileptonic decays $B \to D^{(*)} \ell\,\bar\nu$
(semileptonic tags) to increase the efficiency by sacrificing the 
signal-to-noise ratio.
 
The present $e^+e^-$ $B$-factory experiments are starting to measure
some of these days, as demonstrated by the first evidence of 
$B \to \tau\,\bar \nu$, which was recetly reported by Belle.
However, precision measurements and detection of very difficult modes,
such as $B \to X_s\, \nu\,\bar\nu$, require at least a couple of tens
ab$^{-1}$ data, that can be reached only at the proposed super 
$B$-factories.
  
\subsubsection{$B \to X_s\,\nu\,\bar\nu$}
%\begin{itemize}
%  \item Present status at Belle and BaBar.
%  \item Figure to show the projected sensitivity; 
%        $\Delta {\cal B}(B \to K^{(*)}\, \nu\, \bar\nu)$.
%\end{itemize}

Presently, experimental limits on exclusive $B^- \to X_s \nu \bar\nu$ 
modes are available from Belle and BaBar.
Belle has reported a result of search for the $B^- \to K^- \nu \bar\nu$
decay using a 253 fb$^{-1}$ data sample~\cite{belle_knunu1}.
The analysis utilizes the hadronic tags, and requires that the event 
has no remaining charged tracks nor neutral clusters other than the 
$K^-$ candidate.
FIG\,\ref{fig:Knunu}-a) shows the distribution of remaining neutral
cluster energy recorded in the electromagnetic calorimeter ($E_{ECL}$)
after all the selection cuts are applied.
The signal detection efficiency is estimated to be $43\%$ for the
tagged events.
In the signal region, defined as $E_{ECL} < 0.3$ GeV, the expected number
of signals is 0.70, assuming the Standard Model branching fraction of
${\cal B}(B \to K^- \nu\,\bar\nu) = 4 \times 10^{-6}$, while 
the number of background estimated from the sideband data is $2.6 \pm 1.6$.
The deducued upper limit (90\% C.L.) on the branching fraction is 
${\cal B}(B^- \to K^- \nu \bar\nu) < 3.6 \times 10^{-5}$.
More recently, Belle has reported an upper limit of 
${\cal B}(B^0 \to K^{*0} \nu\,\bar\nu) < 3.4 \times 10^{-4}$,
from a similar analysis on a 492 fb$^{-1}$ data sample~\cite{belle_knunu2}.

BaBar has reported ${\cal B}(B^- \to K^- \nu\,\bar\nu) < 5.2 \times 10^{-5}$,
by combining the hadronic and semileptonic tag events from a 82 fb$^{-1}$ 
data sample~\cite{babar_knunu}.
FIG\,\ref{fig:Knunu}-b) shows the distribution of the remianing energy
($E_{extra}$ in BaBar's notation) for the semileptonic tag sample.
Because of the large $B^- \to D^{(*)} \ell\,\bar\nu$ branching fractions,
the semileptonic tag method has a factor 2 to 3 higher efficiency than the 
hadronic tag method. 

Based on a simple-minded extrapolation from the Belle analysis with the
hadronic tags, the required integrated luminosity for observing the 
$B^- \to K^- \nu\,\bar\nu$ decay with 3(5) $\sigma$ statistical 
significance is 12(33) ab$^{-1}$.
The statistical precision for the branching fraction measurement will 
reach 18\% at 50 ab$^{-1}$.
Addition of the semileptonic tag sample may improve the sensitivity
({\it it is under investigation}).

It is extremely difficult to perform an inclusive search for 
$b \to s \nu \bar\nu$. No serious studies have been made yet.

% --------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=.4\textwidth]{neutrinos/figures/ecl_knunu_belle.eps}
\includegraphics[width=.4\textwidth]{neutrinos/figures/ecl_knunu_babar.eps}
\caption{Distribution of remaining energy for $B^- \to K^- \nu\,\bar\nu$ 
candidates; a) from Belle's analysis using the hadronic tag on a 
253\,fb$^{-1}$ data sample, and b) from BaBar's analysis using the
semileptonic tag on a 82\,fb$^{-1}$ data sample.}
\label{fig:Knunu}
\end{center}   
\end{figure}
% --------------------------------------------------

\subsubsection{$B \to \tau\,\bar\nu$}
%\subsubsubsection{$B \to \tau \nu$}
%\begin{itemize}
%\item Present status at Belle and BaBar
%  \begin{itemize}
%  \item The first evidence of $B \to \tau \nu$ from Belle.
%  \item Figure to show the evidence in the $E_{ECL}$ distribution.
%  \item Figure to show the constraint on charged Higgs in the 
%        $m_H-$tan$\beta$ plane with the present data.
%  \end{itemize}
%\item Extrapolation to higher luminosity
%  \begin{itemize}
%  \item Figure to show the constraint on charged Higgs in the 
%        $m_H-$tan$\beta$ plane with 5 and/or 50ab$^{-1}$ with
%        assumed errors on $f_B$ and $|V_{ub}|$.
%  \item Figure to show the reach in the charged Higgs mass ($m_H$)
%        as a function of the integrated luminosity, at a fixed
%        tan$\beta = 30$ with assumed errors on $f_B$ and $|V_{ub}|$.
%  \end{itemize}
%\end{itemize}

Detection of $B^- \to \tau^-\,\bar\nu$ is very similar to that of 
$B \to K^{(*)} \nu\,\bar\nu$, and it requires that the event has
no extra charged tracks nor neutral clsuters other than those from 
the $\tau$ decay and the accompanying $B$ decay. 

Recently Belle has reported the first evidence of the 
$B^- \to \tau^-\,\bar\nu$ decay by applying the hadronic tag on a 
414\,fb$^{-1}$ data sample~\cite{belle_taunu}.
The reconstructed $\tau$ decay modes are 
$\tau^- \to e^-\,\bar{\nu_e}\,\nu_{\tau}$, 
$\mu^-\,\bar{\nu_{\mu}}\,\nu_{\tau}$, 
$\pi^-\,\nu_{\tau}$, 
$\pi^-\,\pi^0\,\nu_{\tau}$, 
$\pi^-\,\pi^+\,\pi^-\,\nu_{\tau}$.
FIG\,\ref{fig:ecl_taunu}-a) presents the $E_{ECL}$ distribution,
combined for for all the $\tau$ decay modes, which shows an excess of 
events near $E_{ECL} = 0$.
The number of signals ($N_s$) and backgrounds ($N_b$) in the signal
region are determined to be $N_s = 17.2^{+5.3}_{-4.7}$ and 
$N_b = 32.0 \pm 0.7$ by an unbinned maximum likelihood fit.
The significance of the excess is $3.5 \sigma$ including both statistical 
and systematic uncertainties.
The obtained branching fraction is 
${\cal B}(B^- \to \tau^-\,\bar\nu)=
(1.79 ^{+0.56}_{-0.49}\mbox{(sta)} ^{+0.46}_{-0.51}\mbox{(sys)})
\times 10^{-4}$.

BaBar has reported a result of $B^- \to \tau^-\,\bar\nu$ search using
the semileptonic tag on a 288 fb$^{-1}$ data sample~\cite{babar_taunu}.
The tag reconstruction efficiency is about 0.7\%, depending slightly 
on run periods.
When all the analyzed $\tau$ decay modes are combined, 213 events are
observed, while the background is estimated to be $191.7 \pm 11.7$.
Since the excess is not significant, they provide an upper limit of 
${\cal B}(B^- \to \tau^-\,\bar\nu) < 1.8 \times 10^{-4}$ (90\% C.L.), 
and also quote a central value of
${\cal B}(B^- \to \tau^-\,\bar\nu) = (0.88 ^{+0.68}_{-0.67}\mbox{(sta)} 
\pm 0.11 \mbox{(sys)}) \times 10^{-4}$.
The semileptonic tag gives roughly two times higher efficiency 
than the hadronic tag, but introduce more backgrounds. 

Within the context of the Standard Model, the product of the $B$ 
meson decay constant and the magnitude of the CKM matrix element 
$|V_{ub}|$ is determined to be
$f_B |V_{ub}| = (10.1 ^{+1.6}_{-1.4}\mbox{(sta)}
^{+1.3}_{-1.4}\mbox{(sys)}) \times 10^{-4}$\,GeV
from the Belle result.
Using the value of $|V_{ub}|=(4.39 \pm 0.33) \times 10^{-3}$ from
inclusive charmless semileptonic $B$ decay data~\cite{vub},
we obtain $f_B = 0.229 ^{+0.036}_{-0.031}\mbox{(sta)}
^{+0.034}_{-0.037}\mbox{(sta)}$ GeV.
 
The charged Higgs can be constrained by comparing the measured 
branching fraction (${\cal B}^{\rm exp}$) to the Standard 
Model value of ${\cal B}^{SM} = (1.59 \pm 0.40) \times 10^{^4}$, 
which is deduced from the above $|V_{ub}|$ value and 
$f_B = (0.216 \pm 0.022)$\,GeV obtained from lattice QCD calculations
~\cite{lattice_fb}.
Using the Belle result, the ratio is $r_H = 1.13 \pm 0.53$, 
which then constrain the charged Higgs in the $(M_{H^+}, \tan\,\beta)$ 
plane, as shown in FIG\,\ref{fig:higgs_taunu}(top).
The hatched area indicates the region excluded at a confidence level
of 95.5\%.   

Further accumulation of data helps to improve both the statistical
and systematic of the branching fraction.
Some of the major systematic errors, such as ambiguities in the 
reconstruction efficiency and the signal and background shapes, 
come from the limited statistics of a control sample.
On the other hand, the error in the ratio $r_H$ depends on the 
errors in the determination of $|V_{ub}|$ and $f_B$.
FIG\,\ref{fig:higgs_taunu}(bottom) show the expected constraint 
at 5 ab$^{-1}$, assuming the scaling of the experimental error by
$1/\sqrt{L}$ (L is the luminosity) and 5\% relative error for 
both $|V_{ub}|$ and $f_B$.
FIG\,\ref{fig:higgs_taunu_pro} presents the $M_{H^+}$ reach at 
$\tan\,\beta = 30$ as a function of the integrated luminosity.
Here the $M_{H^+}$ reach is defined as the upper limit of the 95.5\% 
excluded region at a given $\tan\,\beta$.
The figure shows expectation for three cases, 
$(\Delta |V_{ub}|/|V_{ub}|,\Delta f_B / f_B) = $
(0\%,0\%), (2.5\%,2.5\%) and (5\%,5\%).
Precise determination of $|V_{ub}|$ and $f_B$ is desired to maximize
the physics reach.

% -------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=.40\textwidth]{neutrinos/figures/ecl_taunu_belle.eps} 
\includegraphics[width=.37\textwidth]{neutrinos/figures/ecl_taunu_babar.eps} 
\caption{Distribution of the remianing energy for $B^- \to \tau^-\,
\bar\nu$ candidates;
a) from Belle's analysis using the hadronic tag on a 414\,fb$^{-1}$ 
data sample, and
b) from BaBar's analysis using the semileptonic tag on a 288\,fb
$^{-1}$ data sample.}
\label{fig:ecl_taunu}
\end{center}   
\end{figure}

% -------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=.4\textwidth]{neutrinos/figures/r_H_taunu_now.eps} 
\includegraphics[width=.4\textwidth]{neutrinos/figures/Mh_tanb_taunu_now.eps} 
\includegraphics[width=.4\textwidth]{neutrinos/figures/r_H_taunu_5ab.eps} 
\includegraphics[width=.4\textwidth]{neutrinos/figures/Mh_tanb_taunu_5ab.eps} 
\caption{
The constraint on the charged Higgs;
$\pm 1\sigma$ boundary in the ratio $r_H$ (left) and the $95.5\%$ C.L. 
exclusion boundaries in the $(M_{H^{+}},\tan\beta)$ plane (right).
The top figures show the constraint from the present Belle result.
The bottom figures show the expected constraints at 5ab $^{-1}$.}
\label{fig:higgs_taunu}
\end{center}   
\end{figure}

% -------------------------------------------------
\begin{minipage}[hbt]{.49\textwidth}
\begin{figure}
\begin{center}
\includegraphics[width=.45\textwidth]{neutrinos/figures/Mh_tanb30_lum_taunu.eps} 
\caption{
Expected $M_{H^+}$ reach at $\tan \beta =30$ as a function of the 
integrated luminosity. The three curves correspond to 
$(\Delta |V_{ub}|/|V_{ub}|,\Delta f_B / f_B) =$
red:(0\%,0\%), blue:(2.5\%,2.5\%) and green:(5\%,5\%).}
\label{fig:higgs_taunu_pro}
\end{center}   
\end{figure}
\end{minipage}
%
\begin{minipage}[hbt]{.49\textwidth}
\begin{figure}
\begin{center}
\includegraphics[width=.6\textwidth]{neutrinos/figures/Mh_tanb_Dtaunu.eps} 
\caption{
Expected constraint on the charged Higgs from measurements of the 
$B \to D \tau\,\bar\nu$ branching fraction at 5 and 50 ab$^{-1}$.
}
\label{higgs_Dtaunu}
\end{center}   
\end{figure}
\end{minipage}

\subsubsection{$B \to D^{(*)} \tau\,\bar\nu$}

The semileptonic $B$ decay into $\tau$ final state, $B \to D^{(*)} \tau\,
\bar\nu$, is also a sensitive probe for the charged Higgs.
In the SM, the branching fractions are expected to be
of the order of $8 \times 10^{-3}$ 
in the Standard Model. Because of the presence of at
least two neutrinos in the final state, the reconstruction of these modes requires the
reconstruction of the other B meson in the event, 
and hence requires a larger data sample with respect to 
that used to measure $B \to D^{(*)} \ell\,\bar\nu$ where $\ell = \mu, \; e$.
Fig~\ref{fig:higgs_Dtaunu} presents the expected constraint in 
the $(M_{H^{+}},\tan\,\beta)$ plane  for a Super $B$ factory with
a 5 and 50~ab$^{-1}$ data sample.

\subsubsection{$B \to \ell \nu$}
%\begin{itemize}
%\item Present status at Belle and BaBar
%  \begin{itemize}
%  \item Analysis without tag
%  \item Analysis with tag (hadronic and semileptonic tags)
%  \end{itemize}
%\item Extrapolation to higher luminosity.
%  \begin{itemize}
%  \item A figure to show $\Delta {\cal B}(B \to \mu \nu)$ and
%  $\Delta R_{\mu\nu/\tau\nu}$ as a function of integrated luminosity.
%  \end{itemize}
%\end{itemize}

Contrary to the $B^- \to \tau\,\bar\nu$ case, the $B^- \to \ell\,\bar\nu$ 
decay has more kinematic constraint because it has only one neutrino 
in the final state, and the charged lepton at a fixed energy in the
$B$ rest frame.
Therefore, present analyses by Belle and BaBar take a conventional
approach, where one looks for a single high momentum lepton, and 
then inclusively reconstruct the accompanying $B$ via a 4-vector sum 
of everything else in the event.
The lepton momentum is smeared in the center-of-mass frame due to $B$
momentum to give a couple of hundred MeV/c width.

Figure~\ref{fig:el_munu}-a) shows the muon momentum distribution 
from the Belle analysis to search for the $B^- \to \mu^-\,\bar\nu$ 
decay using the conventional approach on a 253\,fb$^{-1}$ data sample.
The signal detection efficiency is 2.2\%.
The expected number of signals based on the Standard Model branching 
fraction ($7.1 \times 10^{-7}$) is 4.2, while the estimated background 
is 7.4. 
The reported upper limit is 
${\cal B}(B^- \to \mu^-\,\bar\nu) \leq 1.7 \times 10^{-6}$(90\% C.L.)
~\cite{belle_munu}. 

Recently BaBar has reported a result of the $B \to \mu\,\bar\nu$ search
using the hadronic tags on a 208.7\,fb$^{-}$ data sample.
In this case, as the $B$ momentum is determined by the full reconstruction, 
there is no smearing in the lepton momentum.
Figure~\ref{fig:el_munu}-b) is the muon momentum distribution after all
the selection cuts applied.
The signal detection efficiency is about 0.15\%, an order of magnitude
lower than the conventional analysis.
The reported upper limit is  
${\cal B}(B^- \to \mu^-\,\bar\nu) \leq 7.9 \times 10^{-6}$(90\% C.L.)
~\cite{babar_munu}. 

FIG~\ref{fig:munu_pro} shows the expected statistical significance 
as a function of the integrated luminosity, based on a simple 
extrapolation from the present Belle result.
Accumulation of 1.6\,(4.3) ab$^{-1}$ data will allow us to detect the
$B^- \to \mu^-\,\bar\nu$ signal with 3\,(5) statistical significance.
The 50\,ab$^{-1}$ data at super $B$-factories will allow us to detect
about 800 signals and measure the branching fraction with about 6\% 
statistical precision.

% -------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=.40\textwidth]{neutrinos/figures/el_munu_belle.eps} 
\includegraphics[width=.45\textwidth]{neutrinos/figures/el_munu_babar.eps} 
\caption{
a) Muon momentum distribution from the Belle analysis 
using an inclusive reconstruction of the accompanying $B$
for a 253\,fb $^{-1}$ data sample. 
b) The same distribution from the BaBar analysis using the hadronic
tags on a 208.7 fb$^{-1}$ data sample.
}
\label{fig:el_munu}
\end{center}   
\end{figure}

% -------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=.7\textwidth]{neutrinos/figures/superB_lnu_v3.eps} 
\caption{Expected sensitivity for $B^- \to \mu^-\,\bar\nu$ as a 
function of the integrated luminsoity.}
\label{fig:munu_pro}
\end{center}   
\end{figure}

%\subsubsection{Some notes}

There are some points which need be further studied.
\begin{itemize}

\item Optimization of the tagging; 
there may be some improvement by using the semileptonic tag in 
addition to hadronic tag, especially for $B^- \to K^- \nu\,\bar\nu$, 
for which the impact of additional neutrino seems to be relatively 
small.

\item Effects of backgrounds in high luminosity environment;
future prospect is discussed by extrapolation from the present 
results so far, which may be too simple.
In particular, impact of higher backgrounds to the tagging efficiency
and missing energy resolution have to be more carefully examined.
   
\end{itemize}



==> sll/definitions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Common definitions
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Some shorthand
% turn off italics
\def\ga{\mathrel{\rlap{\raise.6ex\hbox{$>$}}{\lower.6ex\hbox{$\sim$}}}}
\def\la{\mathrel{\rlap{\raise.6ex\hbox{$<$}}{\lower.6ex\hbox{$\sim$}}}}
%\newcommand {\etal}{\mbox{et al.}\xspace} %et al. - no preceeding comma
%\newcommand {\ie}{\mbox{i.e. }\xspace}     %i.e.
%\newcommand {\eg}{\mbox{e.g. }\xspace}     %e.g.
%\newcommand {\etc}{\mbox{etc. }\xspace}     %etc.

% Some software programs
\providecommand{\ALPGEN}{{\sc{alpgen}}\xspace}
\providecommand{\HERWIG}{{\sc{herwig}}\xspace}
\providecommand{\PYTHIA}{{\sc{pythia}}\xspace}
\providecommand{\ISAJET}{{\sc{isajet}}\xspace}
\providecommand{\ISASUGRA}{{\sc{isasugra}}\xspace}
\providecommand{\SHERPA}{{\sc{sherpa}}\xspace}
\providecommand{\GEANT}{{\sc{geant}}\xspace}
\providecommand{\GEANTthree}{{\sc{geant3}}\xspace}
\providecommand{\GEANTfour}{{\sc{geant4}}\xspace}
\providecommand{\GEANE}{{\sc{geane}}\xspace}


% Measurements and units...

\newcommand{\de}{^\circ}
\newcommand{\ten}[1]{\times 10^{#1}}
\newcommand{\unit}[1]{\ensuremath{\mathrm{\;#1}}\xspace}
\newcommand{\mum}{\ensuremath{\mathrm{\;\mu m}}\xspace}
\newcommand{\micron}{\ensuremath{\mathrm{\;\mu m}}\xspace}
\newcommand{\cm}{\ensuremath{\mathrm{\; cm}}\xspace}
\newcommand{\mm}{\ensuremath{\mathrm{\; mm}}\xspace}
\newcommand{\mus}{\ensuremath{\mathrm{\;\mu s}}\xspace}
\newcommand{\keV}{\ensuremath{\mathrm{\; keV}}\xspace}
\newcommand{\MeV}{\ensuremath{\mathrm{\; MeV}}\xspace}
\newcommand{\GeV}{\ensuremath{\mathrm{\; GeV}}\xspace}
\newcommand{\TeV}{\ensuremath{\mathrm{\; TeV}}\xspace}
\newcommand{\keVc}{\ensuremath{\mathrm{\; keV}/c}\xspace}
\newcommand{\MeVc}{\ensuremath{\mathrm{\; MeV}/c}\xspace}
\newcommand{\GeVc}{\ensuremath{\mathrm{\; GeV}/c}\xspace}
\newcommand{\TeVc}{\ensuremath{\mathrm{\; TeV}/c}\xspace}
\newcommand{\keVcc}{\ensuremath{\mathrm{\; keV}/c^2}\xspace}
\newcommand{\MeVcc}{\ensuremath{\mathrm{\; MeV}/c^2}\xspace}
\newcommand{\GeVcc}{\ensuremath{\mathrm{\; GeV}/c^2}\xspace}
\newcommand{\TeVcc}{\ensuremath{\mathrm{\; TeV}/c^2}\xspace}

\newcommand{\pbinv} {\mbox{\ensuremath{\mathrm{\; pb}^{-1}}}\xspace}
\newcommand{\fbinv} {\mbox{\ensuremath{\mathrm{\; fb}^{-1}}}\xspace}
\newcommand{\percms}{\ensuremath{\mathrm{\; cm^{-2}\,s^{-1}}}\xspace}
\newcommand{\lumi}{\ensuremath{{\cal{L}}}\xspace}
%
% Need a convention here:
\newcommand{\LvLow}  {\ensuremath{{\cal{L}}=10^{32}\; \mathrm{cm^{-2}\,s^{-1}}}\xspace}
\newcommand{\LLow}   {\ensuremath{{\cal{L}}=10^{33}\; \mathrm{cm^{-2}\,s^{-1}}}\xspace}
\newcommand{\lowlumi}{\ensuremath{{\cal{L}}=2\times 10^{33}\; \mathrm{cm^{-2}\,s^{-1}}}\xspace}
\newcommand{\LMed}   {\ensuremath{{\cal{L}}=2\times 10^{33}\; \mathrm{cm^{-2}\,s^{-1}}}\xspace}
\newcommand{\LHigh}  {\ensuremath{{\cal{L}}=10^{34}\; \mathrm{cm^{-2}\,s^{-1}}}\xspace}
\newcommand{\hilumi} {\ensuremath{{\cal{L}}=10^{34}\; \mathrm{cm^{-2}\,s^{-1}}}\xspace}

% Some usual physics terms

% SM (still to be classified)

\newcommand{\kt}{\ensuremath{k_{\mathrm{T}}}\xspace}
\newcommand{\BC}{\ensuremath{{B_{\rm c}}}\xspace}
\newcommand{\bbarc}{\ensuremath{{\overline{b}c}}\xspace}
\newcommand{\bbbar}{\ensuremath{{b\overline{b}}}\xspace}
\newcommand{\ccbar}{\ensuremath{{c\overline{c}}}\xspace}
\newcommand{\JPsi}{\ensuremath{{J}/\Psi}\xspace}
%\newcommand{\ttbar}{\ensuremath{{t\overline{t}}}\xspace}
\newcommand{\AFB}{{A_{\rm FB}}\xspace}
\newcommand{\EE}{{e^+e^-}\xspace}
\newcommand{\MM}{{\mu^+\mu^-}\xspace}
\newcommand{\TT}{{\tau^+\tau^-}\xspace}
\newcommand{\wangle}{{sin^{2}\theta_{\rm eff}^{\rm lept}(M^2_{\rm Z})}\xspace}
\newcommand{\ttbar}{\ensuremath{{t\overline{t}}}\xspace}
\newcommand{\stat}{\ensuremath{\mathrm{\; (stat.)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{\; (syst.)}}\xspace}



% Physics symbols ...

\newcommand{\PT}{\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand{\pt}{\ensuremath{p_{\mathrm{T}}}\xspace}
%\newcommand{\ET}{\ensuremath{E_{\mathrm{T}}}\xspace}
\newcommand{\HT}{\ensuremath{H_{\mathrm{T}}}\xspace}
\newcommand{\et}{\ensuremath{E_{\mathrm{T}}}\xspace}
\newcommand{\Em}{\ensuremath{E\!\!\!/}\xspace}
%\newcommand{\ETm}{\ensuremath{{E\!\!\!/}_{\mathrm{T}}}\xspace}
\newcommand{\MET}{\ensuremath{{E\!\!\!/}_{\mathrm{T}}}\xspace}
\newcommand{\Pm}{\ensuremath{p\!\!\!/}\xspace}
\newcommand{\PTm}{\ensuremath{{p\!\!\!/}_{\mathrm{T}}}\xspace}
\newcommand{\ETmiss}{\ensuremath{E_{\mathrm{T}}^{\mathrm{miss}}}\xspace}
\newcommand{\VEtmiss}{\ensuremath{{\vec E}_{\mathrm{T}}^{\mathrm{miss}}}\xspace}
%\newcommand{\Etmiss}{\ensuremath{{E\!\!\!/}_{\mathrm{T}}}\xspace}
%\newcommand{\VEtmiss}{\ensuremath{{{\vec E}\!\!\!/}_{\mathrm{T}}}\xspace}

%%%%%%
%
%
\newcommand{\swsq}{\ensuremath{\sin^2\theta_W}\xspace}
\newcommand{\cwsq}{\ensuremath{\cos^2\theta_W}\xspace}
\newcommand{\tanb}{\ensuremath{\tan\beta}\xspace}
\newcommand{\tanbsq}{\ensuremath{\tan^{2}\beta}\xspace}
\newcommand{\sidb}{\ensuremath{\sin 2\beta}\xspace}
\newcommand{\alpS}{\ensuremath{\alpha_S}\xspace}
\newcommand{\alpt}{\ensuremath{\tilde{\alpha}}\xspace}

\newcommand{\QL}{\ensuremath{Q_L}\xspace}
\newcommand{\sQ}{\ensuremath{\tilde{Q}}\xspace}
\newcommand{\sQL}{\ensuremath{\tilde{Q}_L}\xspace}
\newcommand{\ULC}{\ensuremath{U_L^C}\xspace}
\newcommand{\sUC}{\ensuremath{\tilde{U}^C}\xspace}
\newcommand{\sULC}{\ensuremath{\tilde{U}_L^C}\xspace}
\newcommand{\DLC}{\ensuremath{D_L^C}\xspace}
\newcommand{\sDC}{\ensuremath{\tilde{D}^C}\xspace}
\newcommand{\sDLC}{\ensuremath{\tilde{D}_L^C}\xspace}
\newcommand{\LL}{\ensuremath{L_L}\xspace}
\newcommand{\sL}{\ensuremath{\tilde{L}}\xspace}
\newcommand{\sLL}{\ensuremath{\tilde{L}_L}\xspace}
\newcommand{\ELC}{\ensuremath{E_L^C}\xspace}
\newcommand{\sEC}{\ensuremath{\tilde{E}^C}\xspace}
\newcommand{\sELC}{\ensuremath{\tilde{E}_L^C}\xspace}
\newcommand{\sEL}{\ensuremath{\tilde{E}_L}\xspace}
\newcommand{\sER}{\ensuremath{\tilde{E}_R}\xspace}
\newcommand{\sFer}{\ensuremath{\tilde{f}}\xspace}
\newcommand{\sQua}{\ensuremath{\tilde{q}}\xspace}
\newcommand{\sUp}{\ensuremath{\tilde{u}}\xspace}
\newcommand{\suL}{\ensuremath{\tilde{u}_L}\xspace}
\newcommand{\suR}{\ensuremath{\tilde{u}_R}\xspace}
\newcommand{\sDw}{\ensuremath{\tilde{d}}\xspace}
\newcommand{\sdL}{\ensuremath{\tilde{d}_L}\xspace}
\newcommand{\sdR}{\ensuremath{\tilde{d}_R}\xspace}
\newcommand{\sTop}{\ensuremath{\tilde{t}}\xspace}
\newcommand{\stL}{\ensuremath{\tilde{t}_L}\xspace}
\newcommand{\stR}{\ensuremath{\tilde{t}_R}\xspace}
\newcommand{\stone}{\ensuremath{\tilde{t}_1}\xspace}
\newcommand{\sttwo}{\ensuremath{\tilde{t}_2}\xspace}
\newcommand{\sBot}{\ensuremath{\tilde{b}}\xspace}
\newcommand{\sbL}{\ensuremath{\tilde{b}_L}\xspace}
\newcommand{\sbR}{\ensuremath{\tilde{b}_R}\xspace}
\newcommand{\sbone}{\ensuremath{\tilde{b}_1}\xspace}
\newcommand{\sbtwo}{\ensuremath{\tilde{b}_2}\xspace}
\newcommand{\sLep}{\ensuremath{\tilde{l}}\xspace}
\newcommand{\sLepC}{\ensuremath{\tilde{l}^C}\xspace}
\newcommand{\sEl}{\ensuremath{\tilde{e}}\xspace}
\newcommand{\sElC}{\ensuremath{\tilde{e}^C}\xspace}
\newcommand{\seL}{\ensuremath{\tilde{e}_L}\xspace}
\newcommand{\seR}{\ensuremath{\tilde{e}_R}\xspace}
\newcommand{\snL}{\ensuremath{\tilde{\nu}_L}\xspace}
\newcommand{\sMu}{\ensuremath{\tilde{\mu}}\xspace}
\newcommand{\sNu}{\ensuremath{\tilde{\nu}}\xspace}
\newcommand{\sTau}{\ensuremath{\tilde{\tau}}\xspace}
\newcommand{\Glu}{\ensuremath{g}\xspace}
\newcommand{\sGlu}{\ensuremath{\tilde{g}}\xspace}
\newcommand{\Wpm}{\ensuremath{W^{\pm}}\xspace}
\newcommand{\sWpm}{\ensuremath{\tilde{W}^{\pm}}\xspace}
\newcommand{\Wz}{\ensuremath{W^{0}}\xspace}
\newcommand{\sWz}{\ensuremath{\tilde{W}^{0}}\xspace}
\newcommand{\sWino}{\ensuremath{\tilde{W}}\xspace}
\newcommand{\Bz}{\ensuremath{B^{0}}\xspace}
\newcommand{\sBz}{\ensuremath{\tilde{B}^{0}}\xspace}
\newcommand{\sBino}{\ensuremath{\tilde{B}}\xspace}
\newcommand{\Zz}{\ensuremath{Z^{0}}\xspace}
\newcommand{\sZino}{\ensuremath{\tilde{Z}^{0}}\xspace}
\newcommand{\sGam}{\ensuremath{\tilde{\gamma}}\xspace}
\newcommand{\chiz}{\ensuremath{\tilde{\chi}^{0}}\xspace}
\newcommand{\chip}{\ensuremath{\tilde{\chi}^{+}}\xspace}
\newcommand{\chim}{\ensuremath{\tilde{\chi}^{-}}\xspace}
\newcommand{\chipm}{\ensuremath{\tilde{\chi}^{\pm}}\xspace}
\newcommand{\Hone}{\ensuremath{H_{d}}\xspace}
\newcommand{\sHone}{\ensuremath{\tilde{H}_{d}}\xspace}
\newcommand{\Htwo}{\ensuremath{H_{u}}\xspace}
\newcommand{\sHtwo}{\ensuremath{\tilde{H}_{u}}\xspace}
\newcommand{\sHig}{\ensuremath{\tilde{H}}\xspace}
\newcommand{\sHa}{\ensuremath{\tilde{H}_{a}}\xspace}
\newcommand{\sHb}{\ensuremath{\tilde{H}_{b}}\xspace}
\newcommand{\sHpm}{\ensuremath{\tilde{H}^{\pm}}\xspace}
\newcommand{\hz}{\ensuremath{h^{0}}\xspace}
\newcommand{\Hz}{\ensuremath{H^{0}}\xspace}
\newcommand{\Az}{\ensuremath{A^{0}}\xspace}
\newcommand{\Hpm}{\ensuremath{H^{\pm}}\xspace}
\newcommand{\sGra}{\ensuremath{\tilde{G}}\xspace}
%
\newcommand{\mtil}{\ensuremath{\tilde{m}}\xspace}
%
\newcommand{\rpv}{\ensuremath{\rlap{\kern.2em/}R}\xspace}
\newcommand{\LLE}{\ensuremath{LL\bar{E}}\xspace}
\newcommand{\LQD}{\ensuremath{LQ\bar{D}}\xspace}
\newcommand{\UDD}{\ensuremath{\overline{UDD}}\xspace}
\newcommand{\Lam}{\ensuremath{\lambda}\xspace}
\newcommand{\Lamp}{\ensuremath{\lambda'}\xspace}
\newcommand{\Lampp}{\ensuremath{\lambda''}\xspace}
%
\newcommand{\spinbd}[2]{\ensuremath{\bar{#1}_{\dot{#2}}}\xspace}

%=======
\newcommand{\MD}{\ensuremath{{M_{\rm D}}}\xspace}% ED mass
\newcommand{\Mpl}{\ensuremath{{M_{\rm Pl}}}\xspace}% Planck mass
\newcommand{\Rinv} {\mbox{\ensuremath{{R}^{-1}}}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Personal definitions

%Dirac-Slash (khodjamirian) :
\newcommand{\DS}[1]{/\!\!\!#1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%%% deFazio et al %%%%%%%%%%%%%%%
%--------------------------------------------------------------------------
\def\bold#1{\setbox0=\hbox{$#1$}%
     \kern-.025em\copy0\kern-\wd0
     \kern.05em\%\baselineskip=18ptemptcopy0\kern-\wd0
     \kern-.025em\raise.0433em\box0 }
\def\slash#1{\setbox0=\hbox{$#1$}#1\hskip-\wd0\dimen0=5pt\advance
%\dimen0 by-\ht0\advance\dimen0 by\dp0\lower0.5\dimen0\hbox
         to\wd0{\hss\sl/\/\hss}}
%--------------------------------------------------------------------------
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\nn}{\nonumber}
\newcommand{\dd}{\displaystyle}
\newcommand{\bra}[1]{\left\langle #1 \right|}
\newcommand{\ket}[1]{\left| #1 \right\rangle}
\newcommand{\spur}[1]{\not\! #1 \,}
%--------------------------------------------------------------------------
%--------------------------------------------------------------------------

%%%%%%%%

% Hiller et al
%

\newcommand{\GF}{{G_{\rm F}}}          % Fermi constant constant
\newcommand{\alpem}{{\alpha_{\rm em}}} % QED coupling constant
\newcommand{\Op}{{\cal O}}             % operator
\newcommand{\BR}{{{\cal{B}}}}                 % branching ratio

\newcommand{\Bqll}{{\bar{B}^0_{q} \to \ell^+ \ell^-}}
\newcommand{\Bsmumu}{{\bar{B}^0_{s} \to \MM}}
\newcommand{\BKll}{{\bar{B} \to K \ell^+ \ell^-}}
\newcommand{\BKastll}{{\bar{B} \to K^\ast \ell^+ \ell^-}}
\newcommand{\BKastzeroll}{{\bar{B} \to K^{\ast 0} \ell^+ \ell^-}}
\newcommand{\BKastplusll}{{\bar{B} \to K^{\ast +} \ell^+ \ell^-}}
\newcommand{\BKastgamma}{{\bar{B} \to K^\ast \gamma}}
\newcommand{\BKastKpill}{{\bar{B}^0 \to K^{\ast 0}(\to K^- \pi^+) \ell^+ \ell^-}}

\newcommand{\lsim}{\stackrel{<}{_\sim}}
\newcommand{\gsim}{\stackrel{>}{_\sim}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
